A Quasi-Optimal Spectral Solver for the Heat and Poisson Equations in a Closed Cylinder

We develop a spectral method to solve the heat equation in a closed cylinder, achieving a quasi-optimal $\mathcal{O}(N\log N)$ complexity and high-order, spectral accuracy. The algorithm relies on a Chebyshev--Chebyshev--Fourier (CCF) discretization of the cylinder, which is easily implemented and decouples the heat equation into a collection of smaller, sparse Sylvester equations. In turn, each of these equations is solved using the alternating direction implicit (ADI) method in quasi-optimal time; overall, this represents an improvement in the heat equation solver from $\mathcal{O}(N^{4/3})$ (in previous Chebyshev-based methods) to $\mathcal{O}(N\log N)$. While Legendre-based methods have recently been developed to achieve similar computation times, our Chebyshev discretization allows for far faster coefficient transforms; we demonstrate the application of this by outlining a spectral method to solve the incompressible Navier--Stokes equations in the cylinder in quasi-optimal time. Lastly, we provide numerical simulations of the heat equation, demonstrating significant speed-ups over traditional spectral collocation methods and finite difference methods.

==> 5_NavierStokes.tex <==
\section{Rewriting the Navier--Stokes Equations}

We now have all of the tools at our disposal to rewrite the Navier--Stokes equations as a set of heat equations (with nonlinear forcing terms) in terms of the toroidal and poloidal components of $\vec{\omega}$. 

\begin{theorem}
	Let $\lambda_\omega, \lambda_a, \gamma_\omega, \gamma_a$ be defined as in equations (\ref{PTdefinitions1}) and (\ref{PTdefinitions2}).
	The Navier--Stokes equations can be rewritten in the following way:
	\begin{equation}\label{NSrewrite}
	\left(\frac{\partial}{\partial t} - \frac{1}{Re} \nabla^2 \right)\lambda_\omega = \lambda_a, \qquad \quad \left(\frac{\partial}{\partial t} - \frac{1}{Re} \nabla^2 \right)\gamma_\omega = \gamma_a.
	\end{equation}
\end{theorem}

\begin{proof}
	The primitive form of the incompressible equation is as follows:
	$$
	\left(\frac{\partial}{\partial t} + \vec{v}\cdot\nabla\right)\vec{v} = \frac{1}{Re}\nabla^2\vec{v} -\nabla p,
	$$
	with the additional constraint that $\vec{v}$ is incompressible. Take the curl of both sides of the equation, noting that $\nabla\times\nabla p = 0$ and that the curl commutes with univariate derivatives and the vector Laplacian, and substitute $\vec{\omega} = \nabla\times\vec{v}$ where applicable:
	$$
	\frac{\partial}{\partial t}\vec{\omega} + \nabla\times[\vec{v}\cdot\nabla\vec{v}] = \frac{1}{Re}\nabla^2\vec{\omega}.
	$$
	Using the identity $\frac{1}{2}\nabla(\vec{V}\cdot\vec{V}) = (\vec{V}\cdot\nabla)\vec{V} + \vec{V}\times\nabla\times\vec{V}$,
	$$
	\frac{\partial}{\partial t}\vec{\omega} - \nabla\times[\vec{v}\times\vec{\omega}] = \frac{1}{Re}\nabla^2\vec{\omega}.
	$$
	Now, substitute the PT decompositions in equations (\ref{PTdefinitions1}) and (\ref{PTdefinitions2}):
	\begin{align*}
	\frac{\partial}{\partial t}(\nabla\times[\lambda_\omega \hat{z}] + \nabla\times\nabla\times[\gamma_\omega \hat{z}]) - 
	\frac{1}{Re}\nabla^2(\nabla\times[\lambda_\omega \hat{z}] + &\nabla\times\nabla\times[\gamma_\omega \hat{z}]) \\&= 
	\nabla\times[\lambda_a \hat{z}] + \nabla\times\nabla\times[\gamma_a \hat{z}].
	\end{align*}
	Commute the operators such that the curls are applied last:
	$$
	\nabla\times[\left(\frac{\partial}{\partial t} - \frac{1}{Re} \nabla^2 \right)\lambda_\omega \hat{z}] + \nabla\times\nabla\times[\left(\frac{\partial}{\partial t} - \frac{1}{Re} \nabla^2 \right)\gamma_\omega \hat{z}] = 
	\nabla\times[\lambda_a \hat{z}] + \nabla\times\nabla\times[\gamma_a \hat{z}].
	$$
	The LHS and RHS of this equation represent two different PT decompositions of the same vector field. Because the poloidal and toroidal \emph{vector fields} are unique, this equation can be decoupled:
	$$
	\nabla\times[\left(\frac{\partial}{\partial t} - \frac{1}{Re} \nabla^2 \right)\lambda_\omega \hat{z}] = \nabla\times[\lambda_a \hat{z}],$$
	$$\nabla\times\nabla\times[\left(\frac{\partial}{\partial t} - \frac{1}{Re} \nabla^2 \right)\gamma_\omega \hat{z}] = \nabla\times\nabla\times[\gamma_a \hat{z}].
	$$
	Nonphysical gauge symmetries are available for each scalar component due to the presence of curls. Thus, these equations can be satisfied and these gauge symmetries removed by removing the curls and enforcing that the poloidal and toroidal scalars are the same on each side. Then we retrieve system (\ref{NSrewrite}), which fixes the PT decomposition of $\vec{\omega}$. In turn, this uniquely determines $\vec{\omega}$, but from the Helmholtz Theorem \cite{Zhou2006OnUT}, specifying a vector field's curl and divergence (along with boundary conditions, as detailed in the appendix) uniquely determines that vector field. As $\nabla\cdot\vec{v}=0$ and $\vec{\omega}\equiv\nabla\times\vec{v}$ is also known, $\vec{v}$ is determined.
\end{proof}

Taking $\lambda_\omega, \lambda_a, \gamma_\omega, \gamma_a$ all to be functions of time, our first step in solving the system (\ref{NSrewrite}) is to write these equations as matrix equations.

The $m\times n$ matrix $\mathbf{\Lambda}_{\omega,\ell}(t)$ [resp. $\mathbf{\Gamma}_{\omega,\ell}(t)$] is defined by  $(\mathbf{\Lambda}_{\omega,\ell}(t))_{j,k}=\lambda_\omega^{(j,k,\ell)}$ [resp. $(\mathbf{\Gamma}_{\omega,\ell}(t))_{j,k}=\gamma_\omega^{(j,k,\ell)}$], where $(\lambda_\omega^{(j,k,\ell)})$ [resp. $(\gamma_\omega^{(j,k,\ell)})$] are the interpolation coefficients for $\lambda_\omega$ [resp. $\gamma_\omega$] in CCF$_{(n,m,p)}$. We define $\mathbf{\Lambda}_{a,\ell}(t)$ $\mathbf{\Gamma}_{a,\ell}(t)$ the same way, but for $\lambda_a$ and $\gamma_a$.

Initial conditions $\mathbf{\Lambda}_{\omega,\ell}(0)$ and $\mathbf{\Gamma}_{\omega,\ell}(0)$ can be found by replacing $\vec{V}$ by $\vec{\omega}(r,z,\theta,0)$ in (\ref{PTeq1}) and solving the discretized Poisson equations. The same can be said of $\mathbf{\Lambda}_{a,\ell}(t)$ and $\mathbf{\Gamma}_{a,\ell}(t)$, once $\nabla\times[\vec{v}(t)\times\vec{\omega}(t)]$ is known. To find $\nabla\times[\vec{v}(t)\times\vec{\omega}(t)]$, the following theorem is needed:

\begin{theorem}\label{VectorPotential}
	Let $\vec{\Psi}$ be the vector potential for $\vec{v}$; that is, $\vec{v}=\nabla\times\vec{\Psi}$. If the PT decomposition of $\vec{\Psi}$ is $\vec{\Psi} = \nabla\times[\lambda_\psi \hat{z}] + \nabla\times\nabla\times[\gamma_\psi \hat{z}]$,
	then the following is a decomposition of $\vec{\omega}\equiv\nabla\times\vec{v}$:
	$$
	\vec{\omega} = \nabla\times[-\nabla^2\lambda_\psi \hat{z}] + \nabla\times\nabla\times[-\nabla^2\gamma_\psi \hat{z}].
	$$
\end{theorem}

\begin{proof}
	By taking two curls of the PT decomposition of $\Psi$, it is shown that $\vec{\omega} = \nabla\times\nabla\times\nabla\times[\lambda_\psi \hat{z}] + \nabla\times\nabla\times\nabla\times\nabla\times[\gamma_\psi \hat{z}].$ From the definition of a vector Laplacian, $\nabla\times\nabla\times\vec{V} = \nabla[\nabla\cdot\vec{V}] - \nabla^2\vec{V}$. Under a curl, the gradient term vanishes. Then $\nabla\times\nabla\times\nabla\times\vec{V} = \nabla\times[-\nabla^2\vec{V}]$. Applying this to both sides of the above equation retrieves our desired equality.
\end{proof}

Define $\mathbf{\Gamma}_{\psi,\ell}(t)$ and $\mathbf{\Gamma}_{\psi,\ell}(t)$ the same way we did $\mathbf{\Lambda}_{\omega,\ell}(t)$ and $\mathbf{\Gamma}_{\omega,\ell}(t)$, but for $\lambda_\psi$ and $\gamma_\psi$. We can find $\lambda_\psi$ and $\gamma_\psi$ at any time $t$ using the following discretized Poisson equations:
$$
(RC_{12}D_1+R^2D_2-\ell^2C_{02})\mathbf{\Lambda}_{\psi,\ell}(t)C^T_{02} + R_2\mathbf{\Lambda}_{\psi,\ell}(t)D^T_2 = -R_2\mathbf{\Lambda}_{\omega,\ell}C^T_{02},
$$
$$
(RC_{12}D_1+R^2D_2-\ell^2C_{02})\mathbf{\Gamma}_{\psi,\ell}(t)C^T_{02} + R_2\mathbf{\Gamma}_{\psi,\ell}(t)D^T_2 = -R_2\mathbf{\Gamma}_{\omega,\ell}C^T_{02}.
$$

By taking appropriate curls, $\vec{v}$ and $\vec{\omega}$ can be recovered, and thus $\nabla\times[\vec{v}\times\vec{\omega}]$ can be calculated directly: $\vec{v}=\nabla\times[\gamma_\omega \hat{z}] + \nabla\times\nabla\times[\lambda_\psi \hat{z}]$ and $\vec{\omega}=\nabla\times[\lambda_\omega \hat{z}] + \nabla\times\nabla\times[\gamma_\omega \hat{z}]$. The first equality results from the fact that the curl of the toroidal field of $\vec{A}$ is the poloidal field of $\nabla\times\vec{A}$ for any incompressible $\vec{A}$. From here, we can write the Navier--Stokes equations as a system of discretized heat equations. The system (\ref{NSrewrite}) can be written as follows and solved using the ADI method:
\begin{align*}
\left(R_2-\frac{\kappa^{(b)}}{Re}(RC_{12}D_1+R^2D_2-\ell^2C_{02})\right)\mathbf{\Lambda}_{\omega,\ell}(t+&h)C^T_{02} -\frac{\kappa^{(b)}}{Re}R_2\mathbf{\Lambda}_{\omega,\ell}(t+h)D^T_2 = \\
&R_2\left(\delta^{(b)} \mathbf{\Lambda}_{\omega,\ell}(t)  +\kappa^{(b)}\mathbf{\Lambda}_{a,\ell}(t)\right)C^T_{02},
\end{align*}
\begin{align*}
\left(R_2-\frac{\kappa^{(b)}}{Re}(RC_{12}D_1+R^2D_2-\ell^2C_{02})\right)\mathbf{\Gamma}_{\omega,\ell}(t+&h)C^T_{02}
-\frac{\kappa^{(b)}}{Re}R_2\mathbf{\Gamma}_{\omega,\ell}(t+h)D^T_2 = \\
&R_2\left(\delta^{(b)} \mathbf{\Gamma}_{\omega,\ell}(t)+\kappa^{(b)}\mathbf{\Gamma}_{a,\ell}(t)\right)C^T_{02}.
\end{align*}


==> 8_FutureWork.tex <==
\section{Future Work}
After completion of the incompressible Navier--Stokes solver, the primary goal will be to generalize this work to compressible Navier--Stokes solutions. The general form of the equations is as follows:
$$
\left(\frac{\partial}{\partial t} + \vec{v}\cdot\nabla\right)\vec{v} = \frac{1}{Re}\nabla^2\vec{v} + \frac{1}{3Re}\nabla(\nabla\cdot\vec{v}) - \nabla p + \vec{F},
$$
where the final term, $\vec{F}$, is the \emph{external force} on the fluid. Whether the force is electromagnetic (with conductive fluids), gravitational, or otherwise, it usually takes a very specific form: fundamental forces are all \emph{irrotational}, meaning that the potential energy can be defined.

The best current methods cannot take advantage of this property, though; separating the irrotational component from a vector field leaves behind an \emph{incompressible} component, so any method that decouples the two would require a fast and accurate incompressible Navier--Stokes solver. With the above work on the incompressible equations, though, we can solve for the irrotational component separately. The first advantage of working in this decoupled fashion is that the solution can be found in near optimal time (still $\mathcal{O}(N\log N)$, as this generalization only involves one more forced heat equation). The second advantage is that it allows us to use a much finer discretization with the irrotational component of $\vec{v}$ without sacrificing much-needed algorithm speed.
